Space-time formulation, discretization, and computations for phase-field fracture optimal control problems

The purpose of this work is the development of space-time discretization schemes for phase-field optimal control problems. First, a time discretization of the forward problem is derived using a discontinuous Galerkin formulation. Here, a challenge is to include regularization termsand the crack irreversibility constraint. The optimal control setting is formulated by means of the Lagrangian approach from which the primal part, adjoint, tangent and adjoint Hessian are derived. Herein the overall Newton algorithm is based on a reduced approach by eliminating the state constraint. From the low-order discontinuous Galerkin discretization, adjoint time-stepping schemes are finally obtained. Our algorithmic developments are substantiated and illustrated with some numerical experiments.

==> math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}% Also defined in documentclass siamltex.
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\defsep\colon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\providecommand\tpa[1][0]{^{\tadj{#1}\tpchar}}% Conflict with siamart190516.cls.
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}

